GPT-4 as an Effective Zero-Shot Evaluator for Scientific Figure Captions

There is growing interest in systems that generate captions for scientific figures. However, assessing these systems output poses a significant challenge. Human evaluation requires academic expertise and is costly, while automatic evaluation depends on often low-quality author-written captions. This paper investigates using large language models (LLMs) as a cost-effective, reference-free method for evaluating figure captions. We first constructed SCICAP-EVAL, a human evaluation dataset that contains human judgments for 3,600 scientific figure captions, both original and machine-made, for 600 arXiv figures. We then prompted LLMs like GPT-4 and GPT-3 to score (1-6) each caption based on its potential to aid reader understanding, given relevant context such as figure-mentioning paragraphs. Results show that GPT-4, used as a zero-shot evaluator, outperformed all other models and even surpassed assessments made by Computer Science and Informatics undergraduates, achieving a Kendall correlation score of 0.401 with Ph.D. students rankings

==> table/classifier-table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\centering
\footnotesize
\begin{tabular}{|l|l|ccc|cc|}
\hline
\multirow{3}{*}{\textbf{Model}} & \multirow{3}{*}{\textbf{Data}} & \multicolumn{3}{c|}{\multirow{2}{*}{Reversed Rank}} & \multicolumn{2}{c|}{Reciprocal Rank} \\ \cline{6-7} 
 &  & \multicolumn{3}{c|}{} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Origin\\ Order\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Reversed\\ Order\end{tabular} \\ \cline{3-7} 
 &  & \multicolumn{1}{c|}{\Pearson} & \multicolumn{1}{c|}{\Kendall} & \Spearman & \multicolumn{1}{c|}{\Pearson} & \Pearson \\ \hline
\multirow{2}{*}{\textbf{SciBERT}} & \textbf{Undergrad} & \multicolumn{1}{c|}{AAA} & \multicolumn{1}{c|}{BBB} & CCC & \multicolumn{1}{c|}{DDD} & GGG \\ \cline{2-7} 
 & \textbf{PhD} & \multicolumn{1}{c|}{JJJ} & \multicolumn{1}{c|}{KKK} & LLL & \multicolumn{1}{c|}{MMM} & PPP \\ \hline
\end{tabular}
\end{table*}

==> table/data-cleaning-result-v202306231450.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{@{}lccccc@{}}
\toprule
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Metrics\\ (Norm.)\end{tabular}}} & \multicolumn{5}{c}{\textbf{Data Cleaning Strategy}} \\ \cmidrule(l){2-6} 
 & \multirow{2}{*}{\textbf{No}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}30+\\ Words\end{tabular}}} & \multicolumn{3}{c}{\textbf{Based on GPT-4}} \\ \cmidrule(l){4-6} 
 &  &  & \textbf{L-3} & \textbf{L-4} & \textbf{L-5} \\ \midrule
\textbf{Rouge-1 (F1)} & a.aaa & 1.558 & 1.751 & 1.787 & 1.835 \\
\textbf{Rouge-2 (F1)} & f.fff & 1.777 & 2.194 & 2.276 & 2.256 \\
\textbf{Rouge-L (F1)} & k.kkk & 1.583 & 1.722 & 1.776 & 1.814 \\
\textbf{WMS} & p.ppp & 1.045 & 1.042 & 1.040 & 1.045 \\
\textbf{BERTScore} & u.uuu & 1.081 & 1.122 & 1.125 & 1.131 \\ \midrule
\textbf{Avg. Length} & 1.11 & 38.01 & 11.95 & 12.02 & 12.09 \\ \bottomrule
\end{tabular}
\caption{Caption generation results of different data-cleaning strategies on `Good Quality' beam.}
\end{table}

==> table/main-result-table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\centering
%\footnotesize
\small
\begin{tabular}{|l|l|ccc|ccc|ccc|}
\hline
\multirow{2}{*}{Model} & \multirow{2}{*}{Setting} & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Reversed Rank\\ (Good to Bad:\\ 6, 5, ..., 2, 1)\end{tabular}} & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Reciprocal Rank\\ (Good to Bad:\\ 1/1, 1/2, ..., 1/5, 1/6)\end{tabular}} & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Reversed\\ Reciprocal Rank\\ (Good to Bad:\\ 1/6, 1/5, ..., 1/2, 1/1)\end{tabular}} \\ \cline{3-11} 
 &  & \multicolumn{1}{c|}{\Pearson} & \multicolumn{1}{c|}{\Kendall} & \Spearman & \multicolumn{1}{c|}{\Pearson} & \multicolumn{1}{c|}{\Kendall} & \Spearman & \multicolumn{1}{c|}{\Pearson} & \multicolumn{1}{c|}{\Kendall} & \Spearman \\ \hline
\multirow{4}{*}{\textbf{GPT-4}} & \textbf{Zero-Shot} & \multicolumn{1}{c|}{.501} & \multicolumn{1}{c|}{.401} & .491 & \multicolumn{1}{c|}{.391} & \multicolumn{1}{c|}{.401} & .491 & \multicolumn{1}{c|}{-.492} & \multicolumn{1}{c|}{-.401} & -.491 \\ \cline{2-11} 
 & \textbf{Few-Shot} & \multicolumn{1}{c|}{.531} & \multicolumn{1}{c|}{.429} & .523 & \multicolumn{1}{c|}{.425} & \multicolumn{1}{c|}{.429} & .523 & \multicolumn{1}{c|}{-.513} & \multicolumn{1}{c|}{-.429} & -.523 \\ \cline{2-11} 
 & \textbf{CoT (QA)} & \multicolumn{1}{c|}{.283} & \multicolumn{1}{c|}{.270} & .315 & \multicolumn{1}{c|}{.277} & \multicolumn{1}{c|}{.270} & .315 & \multicolumn{1}{c|}{-.223} & \multicolumn{1}{c|}{-.270} & -.315 \\ \cline{2-11} 
 & \textbf{CoT (QA-YN)} & \multicolumn{1}{c|}{.357} & \multicolumn{1}{c|}{.334} & .400 & \multicolumn{1}{c|}{.324} & \multicolumn{1}{c|}{.334} & .400 & \multicolumn{1}{c|}{-.307} & \multicolumn{1}{c|}{-.334} & -.400 \\ \hline
\multirow{4}{*}{\textbf{GPT-3.5}} & \textbf{Zero-Shot} & \multicolumn{1}{c|}{.465} & \multicolumn{1}{c|}{.370} & .462 & \multicolumn{1}{c|}{.383} & \multicolumn{1}{c|}{.370} & .462 & \multicolumn{1}{c|}{-.433} & \multicolumn{1}{c|}{-.370} & -.462 \\ \cline{2-11} 
 & \textbf{Few-Shot} & \multicolumn{1}{c|}{.462} & \multicolumn{1}{c|}{.371} & .462 & \multicolumn{1}{c|}{.403} & \multicolumn{1}{c|}{.371} & .462 & \multicolumn{1}{c|}{-.402} & \multicolumn{1}{c|}{-.371} & -.462 \\ \cline{2-11} 
 & \textbf{CoT (QA)} & \multicolumn{1}{c|}{.270} & \multicolumn{1}{c|}{.276} & .347 & \multicolumn{1}{c|}{.249} & \multicolumn{1}{c|}{.276} & .347 & \multicolumn{1}{c|}{-.226} & \multicolumn{1}{c|}{-.276} & -.347 \\ \cline{2-11} 
 & \textbf{CoT (QA-YN)} & \multicolumn{1}{c|}{.365} & \multicolumn{1}{c|}{.329} & .404 & \multicolumn{1}{c|}{.317} & \multicolumn{1}{c|}{.329} & .404 & \multicolumn{1}{c|}{-.327} & \multicolumn{1}{c|}{-.329} & -.404 \\ \hline
\multirow{2}{*}{\textbf{Falcon}} & \textbf{Zero-Shot} & \multicolumn{1}{c|}{lll} & \multicolumn{1}{c|}{mmm} & nnn & \multicolumn{1}{c|}{ooo} & \multicolumn{1}{c|}{ppp} & qqq & \multicolumn{1}{c|}{rrr} & \multicolumn{1}{c|}{sss} & ttt \\ \cline{2-11} 
 & \textbf{Few-Shot} & \multicolumn{1}{c|}{uuu} & \multicolumn{1}{c|}{vvv} & www & \multicolumn{1}{c|}{xxx} & \multicolumn{1}{c|}{yyy} & zzz & \multicolumn{1}{c|}{aaaa} & \multicolumn{1}{c|}{bbbb} & cccc \\ \hline
\textbf{Human} & \textbf{Undergrad} & \multicolumn{1}{c|}{.221} & \multicolumn{1}{c|}{.195} & .221 & \multicolumn{1}{c|}{.206} & \multicolumn{1}{c|}{.195} & .221 & \multicolumn{1}{c|}{-.196} & \multicolumn{1}{c|}{-.195} & -.221 \\ \hline
\end{tabular}
\caption{MOVE THE NUMBERS TO THE NEW TABLE}
\end{table*}





%Correlation coefficients (Pearson \Pearson, Kendall \Kendall, and Spearman \Spearman) of model output ratings versus Ph.D. students' assessments, based on different rank conversions: (1) Reversed Rank (high scores indicate high quality), (2) Reciprocal Rank (high scores favor top selections), and (3) Reversed Reciprocal Rank (high absolute scores emphasize detection of low-quality samples).

%\newcommand{\Spearman}{$r_s$\xspace}
%\newcommand{\Kendall}{$\tau$\xspace}
%\newcommand{\Pearson}{$\rho$\xspace}
